The In-Sample Softmax for Offline Reinforcement Learning

Reinforcement learning (RL) agents can leverage batches of previously collected data to extract a reasonable control policy. An emerging issue in this offline RL setting, however, is that the bootstrapping update underlying many of our methods suffers from insufficient action-coverage: standard max operator may select a maximal action that has not been seen in the dataset. Bootstrapping from these inaccurate values can lead to overestimation and even divergence. There are a growing number of methods that attempt to approximate an \emph{in-sample} max, that only uses actions well-covered by the dataset. We highlight a simple fact: it is more straightforward to approximate an in-sample \emph{softmax} using only actions in the dataset. We show that policy iteration based on the in-sample softmax converges, and that for decreasing temperatures it approaches the in-sample max. We derive an In-Sample Actor-Critic (AC), using this in-sample softmax, and show that it is consistently better or comparable to existing offline RL methods, and is also well-suited to fine-tuning.

==> tex/method.tex <==
\section{In-sample Bootstrapping and Kwik Max Optimality}

In this section, we introduce the {knows-what-it-knows (kwik) max optimality} for offline RL. 
We start with a simple bandit problem to illustrate the intuition behind our method, 
then extend to the general RL setting. 


\textbf{A bandit problem}: Assume that the MDP only has one state and $\gamma=0$.  
 Let $\cA = \{1,\dots,K\}$ and $q^*\in\sR^K$ be a reward vector that specifies the reward of each action $a\in\cA$.  
%Given an offline dataset, a value function $q_\theta\approx q$ can be learned.  
As discussed, since $\pi_\dataset$ might not have full coverage over actions, 
 making a greedy decision based on a learned value ${q}\approx q^*$ could be problematic,  especially when the value is an overestimation for  out-of-distribution actions \citep{fujimoto2019offpolicy}. 
To overcome this issue, 
one popular approach is to constrain the learned policy to be similar to  $\pi_\dataset$. 
For example,  consider an objective for $\tau>0$% by considering
\begin{align}
\max_{\pi} \pi \cdot q  - \tau \KL(\pi || \pi_\dataset)\, .
\end{align}
%where $\tau>0$ is a parameter. 
One can immediately observe that  
an optimal policy must be on the support of $\pi_\dataset$: the KL constraint makes sure  $\pi(a) = 0$ as long as $\pi_\dataset(a)=0$ .  
Also, 
it has a closed form solution, $\pi' \propto \pi_\dataset \exp(q / \tau)$. 
One can guarantee $\pi'$ improves $\pi_\dataset$ by realizing that
$
\pi_\dataset\cdot q
%=
%\pi_\dataset\cdot q - \tau \KL(\pi_\dataset || \pi_\dataset) 
\leq 
\pi' \cdot q - \tau \KL(\pi' || \pi_\dataset)
\leq 
\pi' \cdot q
$, 
where the last step follows from the non-negativity of KL divergence. 
Based on this idea many offline RL algorithms are developed \citep{wu2019offlinerl,peng2020advantage,nair2021awac,brandfonbrener2021offline,fujimoto2021mini} \footnote{\citet{fujimoto2021mini} use a \emph{behavior cloning regularization} $(\pi(s) -a)^2$, where $a$ is action in the dataset. We note that this is indeed a KL regularization under Gaussian parameterization with standard deviation. 
}. 
Despite this approach has nice theoretical property and can be easily implemented in practice,  
they do not perform well when $\pi_\dataset$ is sub-optimal, 
since the KL constraint prevents $\pi'$ from exploring more promising regions of the policy space. 
This is confirmed both in previous studies \citep{kostrikov2022offline} and our experiment results {\color{red}TODO}. 


Another solution is to consider an \emph{in-sample} policy optimization, 
\begin{align}
\max_{\pi\preceq \pi_\dataset} \pi\cdot q\, ,
\label{eq:in-sample-po}
\end{align}
which fundamentally avoids selecting an out-of-distribution action. 
The remaining challenge is to design a practical algorithm, since the real $\pi_\dataset$ is not available and one can only estimate it from the data. 
\citet{fujimoto2019offpolicy} propose to approximate the in-sample maximum by taking the maximum over several candidate actions sampled from a learned policy $\pi_\omega\approx\pi_\dataset$. 
On one hand, this method uses a sampling model $\pi_\omega$, which requires strong assumption on $\pi_\cD$.  
More importantly,  
it still cannot avoid bootstrapping from out-of-sample actions due to the error of $\pi_\omega$. 
Recently, \citet{kostrikov2022offline} and \citet{ma2022offline} revisit the in-sample optimization problem and develop algorithms   
 by utilizing expectile regression. 
 Their methods implicitly solve the in-sample maximum without ever querying on out-of-sample actions. 
However, 
since expectile regression does not have a closed form solution, 
there is no convergence guarantee beyond deterministic transition assumption even for the tabular setting. 

Our main contribution is to provide an alternative method to approximate the in-sample maximum based on the \emph{softmax trick}.  
As shown later, 
this new method facilitates practical implementation and enables theoretical convergence guarantee. 
The \emph{softmax}, a smooth approximation to the maximum, is defined as
\begin{align}
\max_{a:\pi_\dataset(a)>0} q(a) 
\approx 
\tau \log \sum_{a:\pi_\dataset(a)>0}  e^{ {q(a)}/{ \tau } } 
%=\tau \log \EE_{a\sim\pi_\dataset} \left[ e^{ {q(a)}/{ \tau } - \log \pi_\dataset(a)}\right]
\, ,
\label{eq:softmax-trick}
\end{align}
where $\tau>0$ controls the degree of approximation. 
In the $\tau \rightarrow 0$ limit one recovers the in-sample maximum.  
We call it \emph{knows-what-it-knows (kwik)-max}, as it is a softmax over actions that are known by $\pi_\dataset$. 
Our first observation is that kwik-max can be approximated using samples by realizing 
 \begin{align}
\tau \log \sum_{a:\pi_\dataset(a)>0}  e^{ {q(a)}/{ \tau } } 
=
\tau \log \EE_{a\sim\pi_\dataset} \left[ e^{ {q(a)}/{ \tau } - \log \pi_\dataset(a)}\right]
\, .
\label{eq:kwik-max-sample-trick}
\end{align}
Note that it only needs samples  from $\pi_\dataset$, which are already provided in the data $\dataset$. 
This totally avoids explicitly querying out-of-distribution actions, 
 bypassing the difficulty of directly implementing \plaineqref{eq:in-sample-po}.  
Our second observation is that kwik-max is the solution of the following \emph{in-sample maximum entropy policy optimization} 
\begin{align}
\tau \log \sum_{a:\pi_\dataset(a)>0}  e^{ {q(a)}/{ \tau } } 
=
\max_{\pi\preceq \pi_\dataset} \pi\cdot q + \tau \sH(\pi)\, ,
\label{eq:kwik-max-me-trick}
\end{align} 
where $\sH$ is the entropy function. 
This builds a nontrival connection to the maximum entropy principle that is widely used in online RL \citep{ziebart2008maximum,mnih2016asynchronous,nachum2017bridging,asadi2017alternative,haarnoja2018soft,mei2019principled,xiao2019maximum}. 
From this perspective, 
kwik-max can also be viewed as a tool for \emph{conservative exploration}: explore to prevent from trapping into a local optimal, while still being suspicious of what it does not know. 
This kind of exploration is especially important when $q$ is a learned value. 
Based on these two observations, in the next section we introduce two practical algorithms for the function approximation setting. 


We now define kwik-max for general RL. 
To avoid bootstrapping from out-of-distribution actions, 
we consider learning a policy that satisfies the \emph{In-sample Bellman optimality equation}
\begin{align}
q_{\pi_\dataset}^*(s,a) = r(s,a) + \gamma \EE_{s'\sim {P}(\cdot|s,a)} \left[ \max_{a': {\pi_\dataset} (a'|s') > 0} q_{\pi_\dataset}^*(s', a')  \right]
\, .
\label{eq:in-sample-bellman}
\end{align}
That is, we aim to satisfy the Bellman optimal consistency only over actions that are in the support of the underline data distribution. 
The \emph{kwik-max optimality equation} is defined as
\begin{align}
\tilde{q}_{\pi_\dataset}^*(s,a) = r(s,a) + \gamma \EE_{s'\sim {P}(\cdot|s,a)} 
\left[ 
\tau \log \sum_{a': {\pi_\dataset} (a'|s') > 0} \exp\Big( \tilde{q}_{\pi_\dataset}^*(s', a')   / \tau \Big)
\right]\, .
\label{eq:in-sample-softmax-bellman}
\end{align}
We have the following key result  showing that kwik-max optimality is a good approximation to the in-sample optimality. 
\begin{theorem}
%$\lim_{\tau\rightarrow 0} \tilde{q}_\beta^* = q_\beta^*$. 
Let $\tilde{q}_{\pi_\dataset}^*$ be the kwik-max optimal value function.
% defined in \plaineqref{eq:in-sample-softmax-bellman}. 
We have $\lim_{\tau\rightarrow 0} \tilde{q}_{\pi_\dataset}^* = q_{\pi_\dataset}^*$. 
Moreover, 
let $\pi_{\pi_\dataset}(a|s) = \sI(a = \argmax_{a: \pi_\dataset(a)>0} q^*_{\pi_\dataset}(s,a) )$ 
be the in-sample optimal policy w.r.t $q^*_{\pi_\dataset}$. 
Define the kwik-max optimal policy,
\begin{align}
\tilde{\pi}_{\pi_\dataset}^*\propto \pi_{\dataset}\exp\left( \frac{\tilde{q}^*_{\pi_\dataset}}{\tau} - \log \pi_\dataset \right)\, .
\end{align}
We have 
$\lim_{\tau \rightarrow \infty} \tilde{\pi}_{\pi_\dataset}^*= \pi_{\pi_\dataset}^*$. 
\label{thm:kwik-optimal-approximation}
\end{theorem}
Due to space limit, the proof of this as well as of all
the remaining results are given in the appendix.

\if0
and 
\begin{align}
\tilde{v}^*_\beta(s) 
 = 
\tau \log
\EE_{a\sim\beta(s)}\left[  \exp\left( \frac{\tilde{q}_\beta^*(s, a)}{ \tau } - \log\beta(a|s) \right)  \right]
\,. 
%\quad
%\tilde{q}^*_\beta(s,a) 
% =
%r(s,a) + \gamma \EE_{s'\sim P(s,a)}\left[ \tilde{v}_\beta^*(s')  \right]\, .
\end{align}
Let $\tilde{\pi}_\beta^*$ be a policy defined as
\begin{align}
\tilde{\pi}_\beta^*(a|s) 
=
\beta(a|s) \exp \left( \frac{\tilde{q}^*_\beta(s,a) - \tilde{v}_\beta^*(s) } {\tau} - \log   \beta(a|s)  \right)\, .
\end{align}
We have $\tilde{v}^*_\beta\rightarrow v^*_\beta$, $\tilde{q}^*_\beta\rightarrow q^*_\beta$  and $\tilde{\pi}_\beta^*\rightarrow \pi_\beta^*$ as $\tau\rightarrow 0$. 
\fi



==> tex/other.tex <==


\section{Headings: first level}

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



==> tex/pseudo.tex <==
%\section{PseudoCode}

\begin{wrapfigure}{L}{0.4\textwidth}
\begin{minipage}{0.4\textwidth}
\begin{algorithm}[H]
	\caption{KWIK AC}\label{alg:insample_pi}
	\begin{algorithmic}
		\FOR {step in $total\_steps$}
		\STATE sample $<s_i, a_i, s'_i, r_i, T_i>$ %from dataset
%		\STATE $L_\omega = -log \pi_\omega(a_i|s_i)$
%		\STATE Update $\pi_\omega$ with $L_\omega$
		\STATE Update $\pi_\omega$ with Eq \ref{eq:mle-loss}
%		\STATE $\hat{a} = \pi_{\psi}(s_i)$
%		\STATE $L_{\phi} = \frac{1}{2}[v_{\phi}(s_i) - (q_{\theta}(s_i, \hat{a}) - \tau * log \pi_{\psi}(\hat{a}|s_i))]^2$
%		\STATE Update $v_{\phi}$ with $L_{\phi}$
		\STATE Update $v_{\phi}$ with Eq \ref{eq:q-loss-inq}
%		\STATE $\hat{a'} = \pi_{\psi}(s'_i)$
%		\STATE $L_{\theta} = \frac{1}{2} [q_{\theta}(s_i, a_i) - (r_i + \gamma (q_{\bar{\theta}}(s'_i, \hat{a'}) - \tau log \pi_{\psi} (\hat{a'}|s'_i)))]^2$
%		\STATE Update $q_{\theta}$ with $L_{\theta}$
		\STATE Update $q_{\theta}$ with Eq \ref{eq:v-loss-inq}
%		\STATE $L_{\psi} = -[exp(\frac{q_{\theta}(s_i, a_i)-v_{\phi}(s_i)}{\tau} - log \pi_\omega(a_i | s_i))) log \pi_\psi(a_i|s_i)]$
%		\STATE Update $\pi_{\psi}$ with $L_{\psi}$
		\STATE Update $\pi_{\psi}$ with Eq \ref{eq:policy-loss}
		\ENDFOR			
	\end{algorithmic}
	\textbf{Return:} $\pi_{\psi}$
\end{algorithm}
\end{minipage}
\end{wrapfigure}

\begin{wrapfigure}{L}{0.4\textwidth}
\begin{minipage}{0.4\textwidth}
\begin{algorithm}[H]
	\caption{KWIK Q-learning}\label{alg:insample_vi}
	\begin{algorithmic}
		\FOR {step in $total\_steps$}
		\STATE sample $<s_i, a_i, s'_i, r_i, T_i>$ %from dataset
%		\STATE $L_\omega = -log \pi_\omega(a_i|s_i)$
%		\STATE Update $\pi_\omega$ with $L_\omega$
		\STATE Update $\pi_\omega$ with Eq \ref{eq:mle-loss}
%		\STATE $L_{\phi} = \frac{1}{2}[v_{\phi}(s_i) - (q_{\bar{\theta}}(s_i, a_i) - \tau log \pi_{\omega}(a_i|s_i))]^2$
%		\STATE Update $v_{\phi}$ with $L_{\phi}$
		\STATE Update $v_{\phi}$ with Eq \ref{eq:v-loss-inac}
%		\STATE $L_{\theta} = \frac{1}{2} [q_{\theta}(s_i, a_i) - (r_i + \gamma v_\phi(s'_i))]^2$
%		\STATE Update $q_{\theta}$ with $L_{\theta}$
		\STATE Update $q_{\theta}$ with Eq \ref{eq:q-loss-inac}
%		\STATE $L_{\psi} = -[exp(\frac{q_{\theta}(s_i, a_i)-v_{\phi}(s_i)}{\tau} - log \pi_\omega(a_i | s_i))) log \pi_\psi(a_i|s_i)]$
%		\STATE Update $\pi_{\psi}$ with $L_{\psi}$
		\STATE Update $\pi_{\psi}$ with Eq \ref{eq:policy-loss}
		\ENDFOR			
	\end{algorithmic}
	\textbf{Return:} $\pi_{\psi}$
\end{algorithm}
\end{minipage}
\end{wrapfigure}


==> tex/related.tex <==
\section{Related Work}

A key challenge of offline reinforcement learning results from the bootstrapping error when estimating temporal difference target by bootstrapping from actions lying out of the offline dataset~\cite{kumar2019stabilizingOQ}. The bootstrapping error can significantly hinder the stability or the optimality of an RL algorithm~\cite{fujimoto2018addressing,kumar2019stabilizingOQ,fujimoto2019offpolicy}. In general, there are three broad perspectives to designing offline RL algorithms by mitigating the effect of bootstrapping errors.  

\textbf{Conservative value estimations.} The first perspective attempts to directly reduce the estimation error by using conservative or pessimistic value estimations for those unseen state-action pairs, observing that those out-of-distribution samples often overestimate action values. The hope is that even though those out-of-distribution actions might still be sampled when estimating the bootstrap targets, their values remain low, so they are less likely to push the value estimates to consistently grow. For example, \cite{kumar2020cql} proposes to estimate an action value’s lower bound, and \cite{kostrikov2021fisherbrc} adopts a special gradient-based regularization on the critic to achieve pessimism estimates. Some work goes step further to learn pessimistic value estimates by leveraging a learned model ~\citep{kidambi2020mbofflinerl,yu2021combo}. 

An alternative way to achieve conservative value estimates is to take some average over different action values~\cite{kumar2019stabilizingOQ,agarwal2020offline,ghasemipour2021emaq}. Hence those OOD action values may have less effect. \cite{wu2021uncertaintyac} detects OOD state-action pairs and down-weights their contribution when estimating training targets. \cite{yang2021implicitofflinemarl} proposes a constraint Q-learning operator, which uses an importance ratio computed by an improved policy and the behavior policy to reweight each action value. \cite{bai2022pessimistic} penalizes Q-values on OOD actions identified by the disagreement of an ensemble of bootstrapped Q-functions. 


\textbf{Behavior regularization.} The second angle to tackle the offline learning challenge is to regularize the learned policy so that it stays close to the behavior policy~\citep{wu2019offlinerl}. While those OOD actions may still get sampled, those incorrect value estimates of the OOD actions can not get frequently updated as those action values being learned stay close to the offline dataset. As a result, these incorrect value estimates are less likely to accumulate to infinite. 
% \cite{zhang2021barcib}
\cite{peng2020advantage} and \cite{nair2021awac} demonstrate that an advantage-weighted regression approach restricts the learned policy to stay close to behavior policy.  \cite{brandfonbrener2021offline} empirically shows that a simple one-step policy improvement---so the learned policy should be close to the behavior policy---yields good performance.  \cite{fujimoto2021mini} shows that an online RL algorithm can be turned into a high-performing offline one by simply adding a behavior cloning term. \cite{yang2022mboffline} regularize the stationary distribution of the learned policy towards the offline data distribution, where the former is estimated using a dynamics model. % \cite{wu2022supportedoffline} explicitly models the support set of behavior policy and then regularizes the learned policy

\textbf{Out of distribution action elimination.} The most straightforward way to avoid bootstrapping error is to eliminate those OOD actions when bootstrapping from actions. However, eliminating OOD actions could be challenging when the state and action spaces are large or continuous. Most existing approaches cannot have a rigorous guarantee of eliminating OOD actions. A popular way to eliminate OOD actions relies on learning a generative model of the offline data~\cite{fujimoto2019offpolicy,zhou2020plas,wu2022supportedoffline}.  \cite{fujimoto2019offpolicy} proposes BCQ (batch constrained q-learning),  relying on a generative model learned from the offline data with the hope that those OOD actions can be avoided when bootstrapping. \cite{zhou2020plas} adopts a similar idea, they learn an action embedding distribution given a state, and an in-distribution action can be sampled with high probability by using a decoder given a state and action embedding. 

Recently, \cite{kostrikov2022offline} considers a state’s value as an action-dependent random variable whose high expectile value can be shown to approximate the max in-distribution action value. Hence they use an expectile regression algorithm to learn the state values learned from offline data, and these state values are further used as targets to learn action values. Hence, bootstrapping from OOD actions can be avoided. \cite{ma2022offline} combines expectile regression and implicit planning to allow flexibly interpolation between Bellman expectation operator (which has the effect of conservative estimates) and the Bellman optimality operator, which encourages learning an optimal policy.  

We would like to mention that these ideas can be naturally correlated and are often combined in algorithmic design. For example, \cite{kumar2019stabilizingOQ} proposes the Bootstrapping Error Accumulation Reduction (BEAR) method, which uses both conservative value estimates when estimating action values and behavior regularization when updating the policy. The critic regularization approach by~\citep{kostrikov2021fisherbrc} theoretically has an effect of regularizing the learned policy towards the behavior policy.

Our work aims at developing a new Bellman operator to eliminate OOD actions when bootstrapping. One should not confuse our work with existing variants of Bellman operators such as the softmax operator, or Mellowmax~\cite{asadi2017mellowmax}, which may have benefits in improving convergence, reducing overestimation error, or enhancing robustness for RL algorithms~\cite{fox2016softupdate,kozuno2019softmax,zhao2019softmax,pan2020softmaxddpg}. Still, they do not restrict bootstrapping to in-distribution actions. 

==> tex/relatedbackup.tex <==
\section{Related Work}

A key challenge of offline reinforcement learning results from the bootstrapping error when estimating temporal difference target by bootstrapping from actions lying out of the offline dataset~\cite{kumar2019stabilizingOQ}. Such bootstrapping error can significantly hinder the stability or the optimality of an RL algorithm~\cite{fujimoto2018addressing,kumar2019stabilizingOQ,fujimoto2019offpollicyrl}. In general, there are three general perspectives to mitigate the effect of bootstrapping error. 

\textbf{Conservative value estimations.} The first perspective attempts to directly reduce the estimation error by using conservative or pessimistic value estimations, observing that those out of distribution actions often result in overestimation of action values. The hope is that, even those out of distribution actions might still be sampled when estimating the bootstrap targets, their values remain low so they are less likely to push the value estimates to consistently grow. 

\textbf{Behavior regularization.} The second angle to tackle the offline learning challenge is to regularize the learned policy so that it stays close to the behavior policy. While those OOD actions may still get sampled, those incorrect value estimates of the OOD actions can not get frequently updated as those action values being learned stay close to the offline dataset. As a result, these incorrect value estimates are less likely accumulated to become larger and larger. \cite{wu2019offlinerl} proposes 

\textbf{Out of distribution action elimination.} The most straightforward way to avoid boostrapping error is to simply not consider those OOD actions at all when boostrapping from actions. However, completely eliminating OOD actions could be a challenging task when we have an extremely large/continuous state and action spaces. Relatively fewer literature is available 

It worths noting that these ideas are often combined in algorithmic design. \cite{kumar2019stabilizingOQ} proposes Bootstrapping Error Accumulation Reduction (BEAR) method, which actually uses both conservative value estimates when estimating action values and behaviour regularization when updating the policy. 

==> tex/setup.tex <==
\section{Preliminaries}

%\paragraph{Markov Decision Process}

%Let $\sR$ be the set of real numbers. 
For a finite set $\cX$, 
we use $\Delta(\cX)$ to denote the set of probability distributions over $\cX$. 
We consider finite Markov Decision Process (MDP) \citep{puterman2014markov} determined by $M=\{\cS, \cA, P, r, \gamma\}$, 
where $\cS$ is a finite state space, $\cA$ is a finite action space, 
%where $\cS$ is the state space, 
%$\cA$ is the action space, 
 $\gamma\in[0, 1)$ is the discount factor, 
$r:\cS\times\cA\rightarrow \sR$ 
and 
$P:\cS\times\cA\rightarrow \Delta(\cS)$ 
are the reward and transition functions. 
For a policy $\pi:\cS\rightarrow \Delta(\cA)$, 
the \emph{value function} specifies the future discounted total reward obtained by following the policy, 
\begin{align}
v^\pi(s) = \EE^\pi\left[ \sum_{t=0}^\infty \gamma^t r(s_t, a_t) \Big| s_0 = s\right]\, ,
\end{align}
where we use $\EE^\pi$ to denote the expectation under the distribution induced by the interconnection of $\pi$ and the environment.  
The \emph{state-action value function}  is defined as
\begin{align}
q^\pi(s,a) = r(s,a) + \gamma \EE_{s'\sim P(\cdot|s,a)} [v^\pi(s')]\, .% \sum\nolimits_{s'} P(s'|s,a) v^\pi(s')\, .
\end{align}
There exists an \emph{optimal policy} $\pi^*$ that maximizes the values for all states $s\in\cS$. 
We use $v^*$ and $q^*$ to denote the optimal value functions. 
It is well-known that 
 the optimal value satisfies the \emph{Bellman optimality equation},
\begin{align}
v^*(s) = \max_a r(s,a) + \gamma \EE_{s'}[v^*(s')]\, ,\quad
q^{*}(s,a) = r(s,a) + \gamma \EE_{s'\sim P(\cdot|s,a)} \left[ \max_{a'} q^{*}(s', a') \right]\, .
\label{eq:bellman-optimality}
\end{align}

\iffalse
\paragraph{Maximum Entropy RL}
The objective of standard RL is to maximize the discounted future return.  
Entropy-regularized RL considers an alternative learning objective \citep{ziebart2008maximum,mnih2016asynchronous,nachum2017bridging,asadi2017alternative,haarnoja2018soft,mei2019principled,xiao2019maximum}, 
which encourages exploration by modifying the value function to
\begin{align}
\tilde{v}^\pi(s)  = v^\pi(s) + \tau \sH(s, \pi)\, ,
\end{align}
where $\tau\geq 0$ is a \emph{temperature} parameter that controls the degree of entropy regularization, 
and the \emph{discounted entropy} $\sH(s,\pi)$ is defined as 
\begin{align}
\sH(s,\pi) =  \EE^\pi\left[ \sum_{t=0}^\infty -\gamma^t \log\pi(a|s) \Big| s_0 = s\right]\, .
\end{align}

\fi


In this work, we consider the problem of learning an optimal decision making policy from a previously collected offline dataset $\dataset = \{s_i, a_i, r_i, s_i'\}^{n-1}_{i=0}$. 
The data is generated by following the following procedure $s_i\sim \rho, a_i\sim\pi_\dataset, s'_i \sim P(\cdot|s_i,a_i), r_i=r(s_i, a_i)$, 
where $\rho$ is a  probability distribution  over states and $\pi_\dataset$ is an \emph{unknown behavior policy}. 
In offline RL, 
the learning algorithm can only take samples from $\dataset$ without further interaction with the environment. 

%Considering $\sI (\cdot)$ to be the indicator function, we define $N(s, a, s') = \sum_{i=0}^{n-1} \sI \left( s_i=s, a_i=a, s'_i = s' \right ), N(s,a) = \sum_{s'} N(s,a,s') $, then the \emph{empirical behavior policy} is defined as $\beta(a|s) = \frac{N(s,a)}{N(s)}$.





